Inflation with Holographic Dark Energy

We investigate the corrections of the holographic dark energy to inflation paradigm. We study the evolution of the holographic dark energy in the inflationary universe in detail, and carry out a model-independent analysis on the holographic dark energy correction to the primordial scalar power spectrum. It turns out that the corrections generically make the spectrum redder. To be consistent with the experimental data, there must be a upper bound on the reheating temperature. We also discuss the corrections due to different choices of the infrared cutoff.

==> makefile <==
all:
	latex HDEInflation.tex
	dvipdf HDEInflation.dvi
	evince HDEInflation.pdf

ver:
	latex HDEInflation.tex
	dvipdf HDEInflation.dvi
	mkdir $(shell date +%R),$(shell date +%F)
	cp HDEInflation.tex $(shell date +%R),$(shell date +%F)/
	cp makefile $(shell date +%R),$(shell date +%F)/
	cp HDEInflation.pdf $(shell date +%R),$(shell date +%F)/
	evince HDEInflation.pdf
clean:
	rm -rf *.aux *.dvi *.log *.pdf *~ *.prv \#*

